Wide and Deep Graph Neural Network with Distributed Online Learning

Graph neural networks (GNNs) are naturally distributed architectures for learning representations from network data. This renders them suitable candidates for decentralized tasks. In these scenarios, the underlying graph often changes with time due to link failures or topology variations, creating a mismatch between the graphs on which GNNs were trained and the ones on which they are tested. Online learning can be leveraged to retrain GNNs at testing time to overcome this issue. However, most online algorithms are centralized and usually offer guarantees only on convex problems, which GNNs rarely lead to. This paper develops the Wide and Deep GNN (WD-GNN), a novel architecture that can be updated with distributed online learning mechanisms. The WD-GNN consists of two components: the wide part is a linear graph filter and the deep part is a nonlinear GNN. At training time, the joint wide and deep architecture learns nonlinear representations from data. At testing time, the wide, linear part is retrained, while the deep, nonlinear one remains fixed. This often leads to a convex formulation. We further propose a distributed online learning algorithm that can be implemented in a decentralized setting. We also show the stability of the WD-GNN to changes of the underlying graph and analyze the convergence of the proposed online learning procedure. Experiments on movie recommendation, source localization and robot swarm control corroborate theoretical findings and show the potential of the WD-GNN for distributed online learning.

==> auxFiles/myTikzDefs.tex <==

% This is a global control on the scale of plots. The constant \myfactor can be defined inside of an individual picture. It is good practice to reset \myfactor to 1 after the end of the picture.
\def\myfactor{1.0}
\def\unit{\myfactor cm}


% This command sets the appearance of axis on pgfplots
\pgfplotsset{ ylabel near ticks,                 % Make x axis label appear close to figure
              xlabel near ticks,                 % Make y axis label appear close to figure
              tick label style = {font=\footnotesize},   % Write numbers in tiny font
              label style = {font=\footnotesize}, % Write axes labels in footnote size font
              title style = {font=\footnotesize},
            }

% Definition of a graph node without filled in color. 
% Controls the appearance of a node in a graph plot
\tikzstyle{empty node} = [ circle, 
                     draw = black,
                     text = black, 
                     minimum size = 0.8*\unit]


% Definition of a graph node. Controls the appearance of a node in a graph plot
\tikzstyle{node} = [ empty node, 
                     fill = blue!50,
                     draw = blue!50,
                     text = white]

\tikzstyle{blue node} = [ empty node, 
                         fill = blue!50,
                         draw = blue!50,
                         text = white]

\tikzstyle{red node} = [ empty node, 
                         fill = red!50,
                         draw = red!50,
                         text = white]

\tikzstyle{green node} = [ empty node, 
                         fill = mygreen!50,
                         draw = mygreen!50,
                         text = white]


\tikzstyle{black node} = [ empty node, 
                           fill = black!40,
                           draw = black!40,
                           text = white]

                         
% Definition of a graph signal dot value without filled in color.
% These are smaller than the nodes and do not allow for text.
% Controls the appearance of a graph signal dot value in a graph plot
\tikzstyle{empty dot} = [ circle, 
                           draw = black,
                           inner sep = 0pt,
                           anchor = center,
                           minimum size = 0.4*\unit]


% Definition of a graph signal dot value.
% Controls the appearance of a graph signal dot value in a graph plot
\tikzstyle{dot} = [ empty dot, 
                    fill = blue!50,
                    draw = blue!50]

\tikzstyle{blue dot} = [ empty dot, 
                         fill = blue!50,
                         draw = blue!50]

\tikzstyle{red dot} = [ empty dot, 
                        fill = red!50,
                        draw = red!50]

\tikzstyle{black dot} = [ empty dot, 
                          fill = black!50,
                          draw = black!50]


% Definition of graph edges. An edge is undirected and doesn't contain arrows. A directed edge has an arrow at the end and a double directed edge contains two arrows. The latter is to be used when we want to emphasize the double directivity.
\tikzstyle{edge}                 = [shorten >=1pt, shorten <=1pt]
\tikzstyle{directed edge}        = [edge, -stealth]
\tikzstyle{double directed edge} = [edge, stealth-stealth]
\tikzstyle{tight edge}                 = [shorten >=0pt, shorten <=0pt]


% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = blue!15,
                      draw = black,
                      text = black]


==> figures/atNode.tex <==
%!TEX root = ../decentralizedWhitePaper.tex

\def \thisplotscale {0.4}
\def \unit {\thisplotscale cm}

\tikzstyle {block} = [draw,
                      rectangle, 
                      fill = blue!10, 
                      minimum height = 2*\unit]

\tikzstyle {long block}  = [block,
                            minimum width = 4*\unit]

\tikzstyle {short block} = [block,
                            minimum width = 2*\unit]

\tikzstyle {circle block}   = [draw,
                            circle,
                            minimum width = 0.9*\unit]

\def\blockDistance{7}


{\footnotesize\begin{tikzpicture}[x = 1*\unit, y=1*\unit, font=\footnotesize]

% Origin
\node at (0,0) (O) {};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw all blocks
%
% Block for aggregator
\path(O) node (zn) {\includegraphics[width=0.2300\textwidth]{figures/AggregationCNNGSLayer1Input.pdf}};
% Block for CNN
\path (zn.east) ++ (\blockDistance,0) node [long block] (CNN) {CNN};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw all arrows
%
% Arrow into CNN
\path [draw, -stealth] (zn.east) -- (CNN.west)  node  [midway, above] (z) {$\bbz_{i}$};
% Arrow out of CNN
\path [draw, -stealth] (CNN.east) -++ (0.5*\blockDistance,0)  node  [midway,above] (outCNN) {$\bbu_{i}$};


\end{tikzpicture}}




==> figures/tikz_styles.tex <==
\tikzstyle{phantom vertex} = [ ellipse, 
                               anchor = center, 
                               minimum height = 0.06*\unit, 
                               minimum width  = 0.06*\unit,
                               inner sep=0pt,
                               anchor=center]
\tikzstyle{red vertex}   = [black, fill = red!20,   phantom vertex, draw]
\tikzstyle{black vertex} = [black, fill = black!20, phantom vertex, draw]
\tikzstyle{blue vertex}  = [black, fill = blue!20,  phantom vertex, draw]
\tikzstyle{green vertex} = [black, fill = green!20,  phantom vertex, draw]
\tikzstyle{vertex}       = [draw, phantom vertex]

\tikzstyle{point} = [ellipse, inner sep=0pt, draw, fill=white, anchor = center,
                     minimum height = 0.05*\unit, minimum width  = 0.05*\unit]
